CoPERLex: Content Planning with Event-based Representations for Legal Case Summarization

Legal professionals often struggle with lengthy judgments and require efficient summarization for quick comprehension. To address this challenge, we investigate the need for structured planning in legal case summarization, particularly through event-centric representations that reflect the narrative nature of legal case documents. We propose our framework, CoPERLex, which operates in three stages: first, it performs content selection to identify crucial information from the judgment; second, the selected content is utilized to generate intermediate plans through event-centric representations modeled as Subject-Verb-Object tuples; and finally, it generates coherent summaries based on both the content and the structured plan. Our experiments on four legal summarization datasets demonstrate the effectiveness of integrating content selection and planning components, highlighting the advantages of event-centric plans over traditional entity-centric approaches in the context of legal judgements.

==> text/tab_app_content.tex <==
\begin{table}[!htb]
\centering
\setlength{\tabcolsep}{3pt} 
\scalebox{0.9}{
\begin{tabular}{lcccccc}
\toprule
\textbf{} & \multicolumn{3}{c}{\textbf{MLS-Long}} & \multicolumn{3}{c}{\textbf{CanLII}} \\ 
\cmidrule(lr){2-4} \cmidrule(lr){5-7} 
         & \textbf{R-1} & \textbf{R-2} & \textbf{R-L} & \textbf{R-1} & \textbf{R-2} & \textbf{R-L} \\ 
Random   & 37.14                   & 16.28                   & 13.71                   & 23.18                   & 3.28                    & 11.69                   \\
BERT-Ext & 42.75                   & 24.81                   & 18.54                   & 23.87                   & 6.78                    & 12.28                   \\
HiBERT   & 44.29                   & 26.27                   & 22.25                   & 24.18                   & 7.12                    & 13.79                   \\
MemSum   & 44.68                   & 26.14                   & 24.15                   & 24.37                   & 7.64                    & 14.55                   \\
Oracle   & 50.99                   & 34.76                   & 36.72                   & 27.23                   & 10.29                   & 16.55          \\ \bottomrule
\end{tabular}}
\caption{Comparison of approaches for the Content Selection component.}
\label{tab:app_content}
\end{table}
